MemServe: Context Caching for Disaggregated LLM Serving with Elastic Memory Pool

Large language model (LLM) serving has transformed from stateless to stateful systems, utilizing techniques like context caching and disaggregated inference. These optimizations extend the lifespan and domain of the KV cache, necessitating a new architectural approach. We present MemServe, a unified system that integrates both inter-request and intra-request optimizations. MemServe introduces MemPool, an elastic memory pool managing distributed memory and KV caches across serving instances. Using MemPool APIs, MemServe combines context caching with disaggregated inference for the first time, supported by a global scheduler that enhances cache reuse through a global prompt tree-based locality-aware policy. Tests show that MemServe significantly improves job completion time and time-to-first-time.

==> note.tex <==
\section{Note}

This section is for notes, it is not part of the paper.

\begin{itemize}
    \item  \Q{Some companies chose FS semantics such as GFS Colossus, Tectonic; some chose append-only semantic such as DFV, WAS. What's the trade-off here?} \A{ (1) from a technical point of a view, FS requires extensive metadata management, and consequently its consistency and fault-tolerance. So a DFS abstraction will be more complex than a pure append-only abstraction. Then, the question falls back to, do all services running on top of DFV build their own metadata manegement layer? If so, is it better to have it in the P layer? We need good answers.}
    
\item
\Q{What services are not a good fit to build on top of DFV, the append-only semantic?}

\item
\Q{Merits of Plog}
\A{(1) Check out the Taurus paper section 3.3. The insight I found is that failure is not transparently handled by the lowest-layer software such as P-layer, but rather exposed to the applications. Fast fail over. This design philosophy was used by several notable networking projects and others.
(2) good for SSDs, wear-leveling etc. (3) comparison to a FS interface, no overuse of metadata.}

\end{itemize}


==> tbl-related-work.tex <==
\begin{table}\footnotesize
    \centering
    \caption{Related Work Comparison} 
    \begin{tabular}{c c  c  c  c }
    \hline
       \scriptsize\bf Work & \scriptsize\bf C. P. & \scriptsize\bf Disagg. P/D & \scriptsize\bf Interference &  \scriptsize\bf Dist-Sched. \\
    \hline
    \hline
       \sysname \  &  \checkmark & \checkmark & \checkmark &  \checkmark \\
    % \hline
       Splitwise\cite{patel2023splitwise} \  &  \scalebox{0.85}{$\times$} &  \checkmark &  \scalebox{0.85}{$\times$} & \checkmark \\

    \hline
    \end{tabular}
    \label{table-related-work}
\end{table}
